Formal Dependability Modeling and Analysis: A Survey

Dependability is an umbrella concept that subsumes many key properties about a system, including reliability, maintainability, safety, availability, confidentiality, and integrity. Various dependability modeling techniques have been developed to effectively capture the failure characteristics of systems over time. Traditionally, dependability models are analyzed using paper-and-pencil proof methods and computer based simulation tools but their results cannot be trusted due to their inherent inaccuracy limitations. The recent developments in probabilistic analysis support using formal methods have enabled the possibility of accurate and rigorous dependability analysis. Thus, the usage of formal methods for dependability analysis is widely advocated for safety-critical domains, such as transportation, aerospace and health. Given the complementary strengths of mainstream formal methods, like theorem proving and model checking, and the variety of dependability models judging the most suitable formal technique for a given dependability model is not a straightforward task. In this paper, we present a comprehensive review of existing formal dependability analysis techniques along with their pros and cons for handling a particular dependability model.

==> README <==
graphbox v1.0
Copyright 2013-2014 Niklas Beisert

graphbox is an extension for the LaTeX2e package 
graphicx to facilitate the placement of graphics
relative to the current position
using additional optional arguments [...]
of \includegraphics. 
For example, changing the vertical alignment is convenient 
for using graphics as elements of (mathematical) formulae. 
Options for shifting, smashing and hiding the graphics 
are mainly intended for designing presentations using, 
e.g., the beamer framework.

The package consists of the files 

    README        readme file
    graphbox.ins  installation file
    graphbox.dtx  source file
    graphbox.sty  package file
    gboxsamp.tex  sample latex file
    gboxsamp.mps  sample graphics file
    graphbox.pdf  manual

The distribution consists of the files README, graphbox.ins and graphbox.dtx.

Run "(pdf)latex graphbox.dtx" to compile the manual graphbox.pdf.

Run "tex graphbox.ins" to create the package graphbox.sty and the sample gboxsamp.tex.
Copy the file graphbox.sty to an appropriate directory of your LaTeX
distribution, e.g. texmf-root/tex/latex/graphbox.

This work may be distributed and/or modified under the
conditions of the LaTeX Project Public License, either version 1.3
of this license or (at your option) any later version.
The latest version of this license is in
  http://www.latex-project.org/lppl.txt
and version 1.3 or later is part of all distributions of LaTeX
version 2005/12/01 or later.

